SQAPlanner: Generating Data-Informed Software Quality Improvement Plans

Software Quality Assurance (SQA) planning aims to define proactive plans, such as defining maximum file size, to prevent the occurrence of software defects in future releases. To aid this, defect prediction models have been proposed to generate insights as the most important factors that are associated with software quality. Such insights that are derived from traditional defect models are far from actionable-i.e., practitioners still do not know what they should do or avoid to decrease the risk of having defects, and what is the risk threshold for each metric. A lack of actionable guidance and risk threshold can lead to inefficient and ineffective SQA planning processes. In this paper, we investigate the practitioners' perceptions of current SQA planning activities, current challenges of such SQA planning activities, and propose four types of guidance to support SQA planning. We then propose and evaluate our AI-Driven SQAPlanner approach, a novel approach for generating four types of guidance and their associated risk thresholds in the form of rule-based explanations for the predictions of defect prediction models. Finally, we develop and evaluate an information visualization for our SQAPlanner approach. Through the use of qualitative survey and empirical evaluation, our results lead us to conclude that SQAPlanner is needed, effective, stable, and practically applicable. We also find that 80% of our survey respondents perceived that our visualization is more actionable. Thus, our SQAPlanner paves a way for novel research in actionable software analytics-i.e., generating actionable guidance on what should practitioners do and not do to decrease the risk of having defects to support SQA planning.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex \
	sections/introduction.tex \
	sections/background.tex \
	sections/studydesign.tex \
	sections/results.tex \
	sections/threats.tex \
	sections/RQ1.tex \
	sections/RQ2.tex 

BIBTEX_FILES = \
	myref.bib

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
# 	open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> sections/relatedwork.tex <==


Software Quality Assurance (SQA) teams play a critical role in the software development process to ensure the absence of software defects. It is not feasible to perform exhaustive SQA tasks (i.e., software testing and code review) on a large software product given the limited SQA resources that are available. Thus, the prioritization of SQA efforts is an essential step in all SQA efforts.



Recently, model-agnostic approaches have been proposed to generate explanations at the prediction level (e.g., LIME [cite], SHAP [cite], BreakDown [cite]).
However, such model-agnostic approaches only provide explanations without the logic involved (i.e., \todo{...}).
Most importantly, recent studies argue that the representation of explanations should be as close as possible to the language of reasoning (i.e., a logic rule) [cite LORE].



Defect models, which identify defect-prone software mod- ules using a variety of software metrics [15, 39, 45], serve two main purposes.


\subsection{Defect Prediction Models}


Defect prediction models play a foundational role in optimising the limited resources of software quality assurance activities, generating quality improvement plans, and validating empirical theories of software quality.
Below, we discuss the literature with respect to the two main purposes of defect models.



\smallsection{Limitation} defect models cannot generate explanations at the instance level


Despite the advances in analytical modelling in software engineering, recent work raises a concern about a lack of explainability of analytical models in software engineering~\cite{dam2018explainable}.
Practitioners also share similar concerns that analytical models in software engineering must be explainable and actionable in order to be of practical use~\cite{dam2018explainable,lewis2013does,menzies2013software}.
For example, Dam~\ea~\cite{dam2018explainable} argue that making software analytics models explainable to software practitioners is as important as achieving accurate predictions.
Lewis~\ea~\cite{lewis2013does} emphasize that defect modelling should be more actionable to help Google engineers debug their programs.
Menzies and Zimmermann~\cite{menzies2013software} also emphasize that software analytics must be actionable.



\subsection{Model-Agnostic Approaches}

Model-agnostic explanations are \todo{....}.
There are two representations of explanations  for model-agnostic approaches.

\subsubsection{Feature-based Model-Agnostic Approaches}

- LIME

- SHAP

- BreakDown

Limitations: No logic \todo{cite LORE} Give example picture

\subsubsection{Rule-based Model-Agnostic Approaches}

- Anchor -> Rules to explain the prediction

- LORE -> Rules to explain the prediction + Counterfactual Explanations (not for every instance)



==> sections/tmp.tex <==
\emph{\textbf{(Step 1)} Designing Granularity Levels of Predictions.} Prior studies have proposed various granularity levels of predictions. 
For example, predicting which components, packages, modules, and files will be defective in the future.
The commonly-focused prediction granularity is at the file level. 

\emph{\textbf{(Step 2)} Designing Software Metrics.} One must determine a set of metrics which operationalize the hypothesis of interest (e.g., using McCabe's Cyclomatic Complexity (CC) to capture code complexity, and the number of field-reported bugs to capture the risk that is associated with a module (bugs)).
There are a variety of software metrics that can be used, for example, code metrics~\cite{menzies2007data} which observe the characteristics of software modules, process metrics~\cite{rahman2013and} which observe the historical development process that involves software modules, and human factors~\cite{Bird2011a} which observe the chracteristics of developers of software modules.

\emph{\textbf{(Step 3)} Designing the Labelling of Software Defects.} One must label software modules as defective if such modules are fixed for a bug report that affected the studied release~\cite{tantithamthavorn2015icse,yathish2019affectedrelease}. 

\emph{\textbf{(Step 4)} Preparing a Defect Dataset.} One must collect software metrics from Version Control Systems (VCSs) and collect the labels of software defects from Issue Tracking Systems (ITSs).

\emph{\textbf{(Step 5)} Developing Defect Models.} Defect models are trained on defect datasets using Artificial Intelligence and Machine Learning (AI/ML) techniques (e.g., logistic regression and random forests).  

\emph{\textbf{(Step 6)} Generating Predictions.} Defect models are applied to testing or unseen datasets to generate predictions.

\emph{\textbf{(Step 7)} Analyzing Defect Models.} Defect models are analyzed using built-in model interpretation techniques (e.g., ANOVA for logistic regression or variable importance for random forests) to understand the overall relationship between the studied metrics and the likelihood of having defects~\cite{jiarpakdee2018impact,tantithamthavorn2018pitfalls}.

\emph{\textbf{(Step 8)} Explaining the Prediction.} Defect models must be explainable by providing justification of the decisions that are made by AI/ML techniques.
However, recent studies raise concerns about a lack of justification of the predictions when applying AI/ML techniques in a software engineering context ~\cite{dam2018explainable}.
For example, when A.java is predicted to be defective with a probability of 0.9, such a probability score only helps developers focus their testing and reviewing effort on the most risky file \textbf{without providing justifications why such file is likely to be defective}.



% For each training dataset, we build defect models using the best classification technique from our preliminary analysis in Section~\ref{sec:best-classifier} (i.e., random forest).
% We use the implementation of random forest that is provided by the scikit-learn Python package.


% \textbf{(Step 1) Select training, testing, and validation data.}
% For each project, we consider the three consecutive releases (i.e., $k-1$, $k$, and $k+1$).
% The first release of that consecutive set is used as training data.
% The second release of that consecutive set is used as testing data, while the third release of that consecutive set is used as validation data.

% \textbf{(Step 2) Build defect models.}


% \textbf{(Step 3) Generate predictions for testing data.}
% We apply the defect models to the testing data to generate the predictions of each instance.

% \textbf{(Step 4) Generate rule-based explanations.}
% For each instance, we apply our framework, LORE, and Anchor to generate rule-based explanations.
% We use the implementation of our framework as described in Section~\ref{sec:methodology}, and use the implementations of LORE and Anchor as described in Section~\ref{sec:baseline}.


% \emph{\textbf{(Step 7)} Analyzing Defect Models.} Defect models are analyzed using built-in model interpretation techniques (e.g., ANOVA for logistic regression or variable importance for random forests) to understand the overall relationship between the studied metrics and the likelihood of having defects~\cite{jiarpakdee2018impact,tantithamthavorn2018pitfalls}.

% \emph{\textbf{(Step 8)} Explaining the Prediction.} Defect models must be explainable by providing justification of the decisions that are made by AI/ML techniques.
% However, recent studies raise concerns about a lack of justification of the predictions when applying AI/ML techniques in a software engineering context ~\cite{dam2018explainable}.
% For example, when A.java is predicted to be defective with a probability of 0.9, such a probability score only helps developers focus their testing and reviewing effort on the most risky file \textbf{without providing justifications why such file is likely to be defective}.


